Three-Body Recombination in Cold Atomic Gases

Systems of three particles show a surprising feature in their bound state spectrum: a series of geometrically scaled states, known as Efimov states. These states have not yet been observed directly, but many recent experiments show indirect evidence of their existence via the so-called recombination process. The theories that predict the Efimov states also predicts either resonant enhancement of the recombination process or suppression by destructive interference, depending on the sign of the interaction between the particles. The theories predict universal features for the Efimov states, for instance that the geometric scaling factor is 22.7, meaning that one state is 22.7 times larger than its lower lying neighbour state. This thesis seeks to investigate non-universal effects by incorporating additional information about the physical interactions into the universal theories.

==> makefile <==
texfile = main.tex

figurefolder = figures
datafolder = data
figuresize = .9,.8

all:figs file

FIGURES=fig3_11\
	#fig2_2 fig2_3 fig2_7\
	fig3_1 fig3_2 fig3_3 fig3_4 fig3_5 fig3_6 fig3_7 fig3_8 fig3_9 fig3_10 fig3_11\
	fig4_1 fig4_2 fig4_4\
	fig5_1 fig5_2 fig5_3 fig5_4 fig5_5\
	fig6_2 fig6_3 fig6_4\

figs:$(FIGURES:=.eps)

%.eps:%.gnu
	@# If a line is commented, then remove the final "\" at the end,
	@# otherwise gnuplot would continue the comment in the rest of the file
	@sed -i 's/^[ \t]*#\(.*\)\\$$/#\1/' $(figurefolder)/$<
	@# If a line starts with d# then delete it completely
	@# Use this when commenting out lines inside a plot
	@sed -i '/^[ \t]*d#/d' $(figurefolder)/$<
	@gnuplot $(figurefolder)/$<
	@# By removing this line, the pdf-document metadata will not be
	@# overwritten by inclusion of the eps-files
	@sed -i"" '/DOCINFO/d' $(figurefolder)/$@

file:$(texfile) 
	latex --shell-escape --synctex=1 $(texfile)
	bibtex $(texfile:.tex=.aux)
	bibtex publications.aux
	dvips $(texfile:.tex=.dvi)
	ps2pdf $(texfile:.tex=.ps)

fig2_2.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set ylabel "Energy" offset 0,1.3;\
	set size 0.7,0.7;\
	unset border;\
	set xzeroaxis lt -1;\
	set yzeroaxis lt -1;\
	set label "Distance" at 3.25,-2;\
	set label "Closed channel" at 2,6;\
	set label "Open channel" at 1,-5.3;\
	set label "$$\\\\epsilon$$" at 3.6,3;\
	set label "$$E$$" at 2,2;\
	set label "$$E^*$$" at .56,2.2;\
	set samples 250;\
	set arrow from 0.21,1.3 to 1.05,1.3 nohead lt 2 lw 3;\
	set arrow from 3.5,0 to 3.5,5 nohead lt 1 lw 4;\
	set noxtics; set noytics;\
	plot [0:4][-13:10] -40*exp(-2*x)+1/x/x t "" lw 3 lc rgb "red", \
	-40*exp(-2*x)+1/x/x+5 t "" lt 1 lw 3 lc rgb "blue", \
	0.75 t "" lt 2 lw 2\
	;' > $(out)

fig2_3.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set key left Left width -4;\
	set size $(figuresize);\
	set lmargin 8;\
	B0=907; dB=0.71;\
	betat=0.103543668186483; act=0.232414125144945; Est=140.479848994506;\
	a1(B)=1-dB/(B-B0);\
	a2(B)=1+betat**2./(sqrt(Est-B*0.134361486697865)-1.0/act-betat**2);\
	set ylabel "$$a[a_{bg}]$$";\
	set xlabel "$$B[G]$$";\
	set xtics add ("$$B_0$$" 907);\
	plot[890:915][0:4]  \
	"data/Na23Feshbach.dat" i 0 t "Experimental data" pt 7 ps .75 w p, \
	"data/Na23Feshbach.dat" i 1 u 1:2:3 t "" lt 1 lw 3 pt 0 w e, \
	a1(x) t "Phenomenological model" lt 1 lw 3 lc rgb "red" w l, \
	a2(x) t "Two-channel model" lt 1 lw 3 lc rgb "blue" w l\
	;' > $(out)

fig2_7.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	data="data/crossing.dat";\
	set xyplane relative 0;\
	set multiplot;\
	unset colorbox;\
	set hidden3d nooffset altdiagonal;\
	set view 45,35;\
	set key at 8,24;\
	set xlabel "Re$$(\\\\rho)$$" offset -3,-1;\
	set ylabel "Im$$(\\\\rho)$$" offset .5,-1;\
	set zlabel "Re$$(\\\\frac{\\\\nu^2}{\\\\rho^2})$$" offset -2;\
	set arrow from 9.2,10.6,0.4 to 9.2,10.6,-0.1 lt 1 lw 3;\
	splot [1:16][0:13][-.5:.5] \
	data i 2 u ($$1/40*20):($$2/26*13):3 matrix t "" lt 1 lc rgb "green" w l, \
	"" i 3 u ($$1/40*20):($$2/26*13):3 matrix t "" lt 1 lc rgb "blue" w l, \
	data i 1 u 1:2:($$3+.001) t "Integration Path" lt 1 lw 6 lc rgb "red" w l, \
	"" i 4 u 1:2:3 t "Branch point, $$\\\\rho_b$$" lt 1 lw 6 lc rgb "black" w l, \
	"" i 0 u 1:(0*$$1):($$2+.003) t "$$n=0$$" lt 1 lw 6 lc rgb "green" w l, \
	"" i 0 u 1:(0*$$1):($$3+.003) t "$$n=1$$" lt 1 lw 6 lc rgb "blue" w l;\
	unset border; unset xtics; unset ztics; set ytics 50;\
	splot [1:16][0:13][-.5:.5] data every 3 i 1 u 1:2:($$3+.001) t "" lt 0 lw 6 lc rgb "red" w l, \
	"" i 4 u 1:2:3 t "" lt 1 lw 6 lc rgb "black" w l, \
	"" every ::::26 i 0 u 1:(0*$$1):($$2+0.003) t "" lt 1 lw 6 lc rgb "red" w l, \
	"" every ::26 i 0 u 1:(0*$$1):($$3+0.003) t "" lt 1 lw 6 lc rgb "red" w l, \
	10 t "" w l\
	;' > $(out)

fig3_1.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set key bottom left Left width -6;\
	set size .9,.8;\
	set xlabel "$$\\\\rho/a$$";\
	set label "$$\\\\nu_0^2(\\\\rho)$$" at graph -0.2,0.5;\
	set arrow from 10,-1.5 to 10,-0.5 lt 1 lw 3 lc rgb "black" nohead;\
	set arrow from 25,-1.5 to 25,-0.5 lt 5 lw 3 lc rgb "black" nohead;\
	set arrow from  1,-1.5 to  1,-0.5 lt 2 lw 3 lc rgb "black" nohead;\
	plot [0:150][-2:0] \
	"data/chap4/eigenvalues.dat" i 0 u 1:2 t "Single-channel zero-range" lt 1 lw 3 lc rgb "red" w l, \
	"" i 0 u 1:4 t "Two-channel" lt 1 lw 3 lc rgb "blue" w l, \
	"" i 0 u 1:6 t "Effective range expansion" lt 1 lw 3 lc rgb "green" w l, \
	"" i 0 u 1:8 t "" lt 5 lw 3 lc rgb "blue" w l, \
	"" i 0 u 1:10 t "" lt 5 lw 3 lc rgb "green" w l, \
	"" i 1 u 1:2 t "" lt 2 lw 3 lc rgb "blue" w l, \
	"" i 1 u 1:4 t "" lt 2 lw 3 lc rgb "green" w l;\
	set size 0.45,0.445;\
	set origin 0.45,0.355;\
	set xlabel ""; set ylabel "";\
	set ytics (-2,-4,-6,-8,-10);\
	set xtics (0,200,400,600,800);\
	unset label 1;\
	unset arrow 1;\
	unset arrow 2;\
	unset arrow 3;\
	set label "$$\\\\nu_0^2(\\\\rho)$$" at graph -0.4,0.5;\
	plot [0:1000][-10:0] \
	"data/chap4/eigenvalues.dat" i 0 u 1:2 t "" lt 1 lw 3 lc rgb "red" w l, \
	"" i 0 u 1:4 t "" lt 1 lw 3 lc rgb "blue" w l, \
	"" i 0 u 1:6 t "" lt 1 lw 3 lc rgb "green" w l, \
	"" i 0 u 1:8 t "" lt 2 lw 5 lc rgb "blue" w l, \
	"" i 0 u 1:10 t "" lt 2 lw 5 lc rgb "green" w l;\
	;' > $(out)

fig3_2.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set size 0.9,0.6;\
	set key bottom right width -6;\
	set xlabel "$$\\\\rho/a_0$$";\
	set label 1 "$$\\\\nu_0^2(\\\\rho)$$" at graph -0.2,0.5 ;\
	plot[0:30][-1.4:-0.7]  \
	"data/lambdadata2" i 0 u 1:($$2+4) t "Single-channel zero-range" lt 2 lw 3 lc rgb "red" w l, \
	"" i 1 u 1:($$2+4) t "Two-channel" lt 1 lw 3 lc rgb "blue" w l, \
	"" i 2 u 1:($$2+4) t "Effective range expansion, $$R_0=-5a_0$$" lt 5 lw 3 lc rgb "green" w l, \
	"" i 3 u 1:($$2+4) t "Effective range expansion, $$R_0=+5a_0$$" lt 0 lw 3 lc rgb "magenta" w l, \
	0 t "" ;\
	;' > $(out)

fig3_3.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set key bottom center Left width -6 spacing 1.3;\
	set object 1 polygon from 1.0,-0.975 to 0.975,-0.975 to 1.0,-1.0;\
	set object 1 fc rgb "#dddddd" fillstyle solid 1.0;\
	set xlabel "$$\\\\textrm{sign}(a)\\\\times\\\\left\\\\vert\\\\dfrac{a_0^2}{a^2}\\\\right\\\\vert^{1/8}$$";\
	set ylabel "$$-\\\\left\\\\vert E_T^{(n)}\\\\dfrac{2ma_0^{2}}{\\\\hbar^2}\\\\right\\\\vert^{1/8}$$";\
	set label "$$n=1$$"   at -0.10,-0.67;\
	set label "$$n=2$$"   at -0.10,-0.38;\
	set label "$$n=3$$"   at -0.10,-0.20;\
	set label "$$a_2^*$$" at  0.20,-0.60;\
	set label "$$a_3^*$$" at  0.20,-0.47;\
	set arrow from 0.30,-0.60 rto 0.2,0.05 lt 1 lw 3 lc rgb "black";\
	set arrow from 0.24,-0.42 rto 0.0,0.15 lt 1 lw 3 lc rgb "black";\
	X(a)=sgn(a)*(sgn(a)*a)**-0.25;\
	Y(E)=sgn(E)*(sgn(E)*E)**(1.0/8);\
	R0=-5;\
	R(a)=R0*(1-1/a)**2;\
	Ed(a)=-1/R(a)**2*(1-sqrt(1-2*R(a)/a))**2;\
	set label "$$a^{(-)}$$" at -0.925,-0.77;\
	set arrow from -0.87,-0.7 to -0.87,-0.55;\
	plot[-1:1][-1.1:0] \
	"data/efimovPlotData" i 0 u (X($$1)):(Y($$2)) t "Single-channel zero-range" lt 1 lw 3 lc rgb "red" w l, \
	"" i 1 u (X($$1)):(Y($$2)) t "" lt 1 lw 3 lc rgb "red" w l, \
	"" i 2 u (X($$1)):(Y($$2)) t "" lt 1 lw 3 lc rgb "red" w l, \
	"" i 3 u (X($$1)):(Y($$2)) t "Two-channel" lt 1 lw 3 lc rgb "blue" w l, \
	"" i 4 u (X($$1)):(Y($$2)) t "" lt 1 lw 3 lc rgb "blue" w l, \
	"" i 5 u (X($$1)):(Y($$2)) t "" lt 1 lw 3 lc rgb "blue" w l, \
	"" i 6 u (X($$1)):(Y($$2)) t "Effective range expansion" lt 1 lw 3 lc rgb "green" w l, \
	"" i 7 u (X($$1)):(Y($$2)) t "" lt 1 lw 3 lc rgb "green" w l, \
	"" i 8 u (X($$1)):(Y($$2)) t "" lt 1 lw 3 lc rgb "green" w l, \
	"" i 3 every ::77 u (X($$1)):(Y($$3)) t "" lt 2 lw 3 lc rgb "blue" w l, \
	-(-Ed(x**-4))**(1.0/8)*sgn(x) t "" lt 2 lw 3 lc rgb "#dddddd" w filledcurves y2, \
	-(-Ed(x**-4))**(1.0/8)*sgn(x) t "" lt 2 lw 3 lc rgb "green" w l, \
	-x t "" lt 2 lw 3 lc rgb "red";\
	;' > $(out)

fig3_4.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set key Left width -6 spacing 1.3;\
	set xlabel "$$R_0/a_0$$";\
	set ylabel "$$\\\\kappa^*a^{(-)}$$";\
	plot[-2:2][-1.9:-1] \
	"+" u ($$1*0):(-1.9+(-1.3+1.9)*($$1+2)/4.0) t "" lt 1 lw 1 lc rgb "grey" w l, \
	-1.46887119951675 t "Single-channel zero-range" lt 1 lw 3 lc rgb "red", \
	"data/chap4/twochdata0.5" i 0 u ($$1):($$2*$$3) t "Two-channel" lt 1 lw 3 lc rgb "blue" w l, \
	"data/chap4/twochdata0.6" i 0 u ($$1):($$2*$$3) t "" lt 1 lw 3 lc rgb "blue" w l, \
	"data/chap4/twochdata0.7" i 0 u ($$1):($$2*$$3) t "" lt 1 lw 3 lc rgb "blue" w l, \
	"data/chap4/effRdata0.5" i 0 u ($$1):($$2*$$3) t "Effective range expansion" lt 1 lw 3 lc rgb "green" w l, \
	"data/chap4/effRdata0.6" i 0 u ($$1):($$2*$$3) t "" lt 1 lw 3 lc rgb "green" w l, \
	"data/chap4/effRdata0.7" i 0 u ($$1):($$2*$$3) t "" lt 1 lw 3 lc rgb "green" w l;\
	;' > $(out)

fig3_5.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set key Left width 0 spacing 1.3;\
	set xlabel "$$R_0/a_0$$";\
	set ylabel "$$\\\\sqrt{E_T^{(n*)}/E_T^{(n+1*)}}$$";\
	plot[-5:3][21:27] 22.7 t "" lt 1 lw 3 lc rgb "black", \
	"data/chap4/energyRatiosAtResonanceData" i 0 t "$$r_c=0.1$$" lt 1 lw 3 lc rgb "red" w l, \
	"" i  1 t "" lt 2 lw 3 lc rgb "red" w l, \
	"" i  2 t "$$r_c=0.07$$" lt 1 lw 3 lc rgb "yellow" w l, \
	"" i  3 t "" lt 2 lw 3 lc rgb "yellow" w l, \
	"" i  4 t "$$r_c=0.05$$" lt 1 lw 3 lc rgb "blue" w l, \
	"" i  5 t "" lt 2 lw 3 lc rgb "blue" w l, \
	"" i  6 t "$$r_c=0.1$$" lt 1 lw 3 lc rgb "green" w l, \
	"" i  7 t "" lt 2 lw 3 lc rgb "green" w l, \
	"" i  8 t "$$r_c=0.07$$" lt 1 lw 3 lc rgb "cyan" w l, \
	"" i  9 t "" lt 2 lw 3 lc rgb "cyan" w l, \
	"" i 10 t "$$r_c=0.05$$" lt 1 lw 3 lc rgb "magenta" w l, \
	"" i 11 t "" lt 2 lw 3 lc rgb "magenta" w l, \
	"" i 12 t "" lt 1 lw 3 lc rgb "cyan" w l, \
	"" i 13 t "" lt 1 lw 3 lc rgb "cyan" w l, \
	"" i 14 t "" lt 1 lw 3 lc rgb "green" w l, \
	"" i 15 t "" lt 1 lw 3 lc rgb "green" w l, \
	"" i 16 t "" lt 1 lw 3 lc rgb "magenta" w l, \
	"" i 17 t "" lt 1 lw 3 lc rgb "magenta" w l, \
	0 t "" lt 1 lw 3 lc rgb "black" w l;\
	;' > $(out)

fig3_6.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set key left Left width -6;\
	set size 1,.9;\
	set key spacing 1.3;\
	set lmargin 8;\
	factor=9.08828e-29/25**4;\
	set xlabel "$$a/a_0$$";\
	set ylabel "$$\\\\rec/(\\\\textrm{cm}^6\\\\textrm{s}^{-1})$$";\
	set label 1 "$$a_1^*$$" at 110,1e-24;\
	set label 2 "$$a_2^*$$" at 2400,1e-20;\
	set arrow 3 from 119,1e-25 to 119,1e-27;\
	set arrow 4 from 2676,1e-21 to 2676,1e-23;\
	set logscale x; set logscale y;\
	set format x "$$10^%L$$";\
	set format y "$$10^{%L}$$";\
	set multiplot;\
	plot[47:][] \
	"data/chap4/Defaultrecombination_single" i 0 u 1:($$2*factor) t "Single-channel zero-range" lt 1 lw 3 lc rgb "red" w l, \
	"data/chap4/Defaultrec_multi-3" i 0 u ($$1):($$2*factor) t "" lt 3 lw 3 lc rgb "blue" w l, \
	"data/chap4/Defaultrec_multi-10" i 0 u ($$1):($$2*factor) t "Two-channel" lt 1 lw 3 lc rgb "blue" w l, \
	"data/chap4/Defaultrec_ERE-3" i 0 u ($$1):($$2*factor) t "" lt 2 lw 3 lc rgb "green" w l, \
	"data/chap4/Defaultrec_ERE-10" i 0 u ($$1):($$2*factor) t "Effective range expansion" lt 1 lw 3 lc rgb "green" w l;\
	set size 0.55,0.4;\
	set origin 0.4,0.125;\
	set xlabel ""; set ylabel "";\
	unset label 1;unset label 2;unset arrow 3;unset arrow 4;\
	set ytics (1e-33,1e-31,1e-29,1e-27);\
	set xtics (80,110,150,200);\
	set format x "%g";\
	plot[80:200][1e-33:1e-26] \
	"data/chap4/Defaultrecombination_single" i 0 u 1:($$2*factor) t "" lt 1 lw 3 lc rgb "red" w l, \
	"data/chap4/Defaultrec_multi-3" i 0 u ($$1):($$2*factor) t "" lt 3 lw 3 lc rgb "blue" w l, \
	"data/chap4/Defaultrec_multi-10" i 0 u ($$1):($$2*factor) t "" lt 1 lw 3 lc rgb "blue" w l, \
	"data/chap4/Defaultrec_ERE-3" i 0 u ($$1):($$2*factor) t "" lt 2 lw 3 lc rgb "green" w l, \
	"data/chap4/Defaultrec_ERE-10" i 0 u ($$1):($$2*factor) t "" lt 1 lw 3 lc rgb "green" w l;\
	;' > $(out)

fig3_7.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set key bottom Left spacing 1.3 width -6;\
	set xlabel "$$R_0/a_0$$";\
	set label 1 "$$\\\\dfrac{a_2^*}{a_1^*}$$" at graph -0.2, graph 0.5;\
	plot[-12:0][18:] \
	0*x+22.7 t "Single-channel zero-range" lt 1 lw 3 lc rgb "red" w l, \
	"data/chap4/Amin_Reff" i 1 u 1:(2676/$$2) t "Two-channel" lt 1 lw 3 lc rgb "blue" w l, \
	"" i 0 u 1:(2676/$$2) t "Effective range expansion" lt 1 lw 3 lc rgb "green" w l;\
	;' > $(out)

fig3_8.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set key left Left width -2;\
	set size $(figuresize);\
	set lmargin 8;\
	set xlabel "$$a/a_0$$";\
	set ylabel "$$\\\\rec/(\\\\text{cm}^6\\\\text{s}^{-1})$$";\
	factor = 7.10030436074426e-35*1e2;\
	set label "$$a_1^*$$" at 60,3e-25;\
	set label "$$a_2^*$$" at 967,1e-27;\
	set label "$$\\\\dfrac{a_ 2^*}{a_1^*}\\\\approx15.7$$" at 175,1e-29;\
	set arrow 1 from 62,1e-25 to 62,1e-27;\
	set arrow 2 from 967,5e-27 to 967,5e-25;\
	set arrow 3 from 61.69,1e-30 to 967,1e-30 heads;\
	set logscale x;set logscale y; set format y "$$10^{%L}$$";\
	plot[20:2e3][1e-31:]\
	"data/chap5/Na23rec.dat" u 1:($$2*1e-30) t "$${}^{23}$$Na data" pt 7 ps .75 w p,\
	"data/chap5/Na23rec.dat" i 1 u 1:($$2*1e-30):($$3*1e-30) t "" lt 1 lw 3 pt 0 w e,\
	"data/chap5/moreNa23rec" u 1:($$2*factor) t "Two-channel" lt 1 lw 3 lc rgb "blue" w l,\
	x**4*factor/20 t "$$a^4$$ scaling" lt 2 lw 3 lc rgb "red"\
	;' > $(out)

fig3_9.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set key left Left width -2;\
	set size $(figuresize);\
	set lmargin 8;\
	set xlabel "$$a/a_0$$";\
	set ylabel "$$\\\\rec/(\\\\text{cm}^6\\\\text{s}^{-1})$$";\
	factor = 1.22984505922203e-47;\
	set label "$$a_1^*$$" at 200,1e-24;\
	set label "$$a_2^*$$" at 4070,1e-27;\
	set label "$$\\\\dfrac{a_ 2^*}{a_1^*}\\\\approx22.7$$" at 700,7e-28;\
	set arrow 1 from 210,5e-25 to 210,5e-27;\
	set arrow 2 from 4770,5e-27 to 4770,5e-25;\
	set arrow 3 from 210,1e-28 to 4770,1e-28 heads;\
	set logscale x;set logscale y; set format y "$$10^{%L}$$";\
	plot[60:6500][:1e-20]  \
	"data/chap5/Cs133rec.dat" u 1:($$2*1e12) t "$${}^{133}$$Cs data" pt 7 ps .75 w p, \
	"data/chap5/Cs133rec" u 1:($$3*1e12) t "Two-channel" lt 1 lw 3 lc rgb "blue" w l, \
	"data/chap5/Cs133sigma.dat" u 1:($$2*1e12) t "" lt 1 lc rgb "black" w l, \
	x**4*factor/20*1e12 t "$$a^4$$ scaling" lt 2 lw 3 lc rgb "red";\
	;' > $(out)
	
fig3_10.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set key left Left width -2;\
	set size $(figuresize);\
	set lmargin 8;\
	set xlabel "$$a/a_0$$";\
	set ylabel "$$\\\\rec/(\\\\text{cm}^6\\\\text{s}^{-1})$$";\
	factor = 4.18939479561083e-35;\
	set label "$$a_1^*$$" at 224,1e-22;\
	set label "$$a_2^*$$" at 5050,3e-27;\
	set label "$$\\\\dfrac{a_ 2^*}{a_1^*}\\\\approx22.2$$" at 600,3e-28;\
	set arrow 1 from 254.2,5e-24 to 254.2,5e-26;\
	set arrow 2 from 5645,1e-26 to 5645,1e-24;\
	set arrow 3 from 254.2,1e-29 to 5645,1e-29 heads;\
	set logscale x; set logscale y;\
	set format x "$$10^{%L}$$"; set format y "$$10^{%L}$$";\
	plot[17:3e4][] \
	"data/chap5/K39rec.dat" i 0 u ($$1):($$2) t "$${}^{39}$$K data" pt 7 ps .75 lc rgb "black" w p, \
	"data/chap5/K39sigma.dat" t "" lt 1 lc rgb "black" w l, \
	"data/chap5/K39rec" i 0 u ($$1):($$3*factor) t "Two-channel" lt 1 lw 3 lc rgb "blue" w l, \
	x**4*factor/20 t "$$a^4$$ scaling" lt 2 lw 3 lc rgb "red";\
	;' > $(out)

fig3_11.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set key left Left width -2;\
	set size $(figuresize);\
	set lmargin 8;\
	set xlabel "$$a/a_0$$";\
	set ylabel "$$\\\\rec/(\\\\text{cm}^6\\\\text{s}^{-1})$$";\
	factor = 2.32659983070990e-34*2;\
	s0=1.00624;\
	as=119;\
	f(a) = 1.5e-37*128*pi**2*(4*pi-3**1.5)*sin(s0*log(a/as))**2/(sinh(pi*s0)**2+cos(s0*log(a/as)**2))*a**4;\
	set label "$$a_1^*$$" at 119,5e-24;\
	set label "$$a_2^*$$" at 2376,3e-27;\
	set label "$$\\\\dfrac{a_ 2^*}{a_1^*}\\\\approx21.4$$" at 300,2e-28;\
	set arrow 1 from 124.8,1e-24 to 124.8,1e-26;\
	set arrow 2 from 2674,1e-26 to 2674,1e-24;\
	set arrow 3 from 124.8,1e-29 to 2674,1e-29 heads;\
	set logscale x; set logscale y;\
	set format x "$$10^{%L}$$"; set format y "$$10^{%L}$$";\
	plot[20:1e4][] \
	"data/chap5/Li7rec.dat" t "$${}^7$$Li data" pt 7 ps .5 lc rgb "black" w p, \
	"data/chap5/Li7sigma.dat" t "" lt 1 lc rgb "black" w l, \
	"data/chap5/Li7rec" i 0 u ($$1):($$3*factor) t "Two-channel" lt 1 lw 3 lc rgb "blue" w l, \
	x**4*factor/20 t "$$a^4$$ scaling" lt 2 lw 3 lc rgb "red";\
	;' > $(out)

fig4_1.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set key right bottom Left width -7;\
	abar =  0.955977594972250;\
	set xlabel "$$\\\\log_{10}(s_\\\\text{res})$$";\
	set ylabel "$$\\\\vdW/a^{(-)}$$";\
	f(x,rc) = -abar/31.756/rc;\
	set label "$${}^7$$Li" at -0.4,0.0;\
	set label "$${}^{39}$$K" at 0.2,0.0;\
	set label "$${}^{85}$$Rb" at 1.1,0.0;\
	set label "$${}^{133}$$Cs" at 2.30,0.0;\
	set arrow from 2.15 ,-0.035 to 3.25 ,-0.035 heads size .05,90;\
	plot[-2:3.5][-.65:.05] \
	"data/AminusReffDependence" i 1 u (column(1)*4+1):(f(column(1),column(2))) t "Single-channel zero-range" lt 2 lw 3 lc rgb "red" w l, \
	for [i=3:10] "" i 1 u (column(1)*4+1):(f(column(1),column(i))) t "" lt 2 lw 3 lc rgb "red" w l, \
	"" i 0 u (log10(-1/$$1)):(1/$$2) t "Two-channel" lt 1 lw 3 lc rgb "blue" w l, \
	for [i=3:10] "" i 0 u (log10(-1/$$1)):(1/column(i)) t "" lt 1 lw 3  lc rgb "blue" w l, \
	"data/AtomicData" every ::0::0  u (log10($$1/abar)):($$2/$$3) t "" pt 5 ps 1.5 lc rgb "green" w p, \
	"" every ::1::1  u (log10($$1/abar)):($$2/$$3) t "" pt 7 ps 1.5 lc rgb "black" w p, \
	"" every ::2::2  u (log10($$1/abar)):($$2/$$3) t "" pt 9 ps 1.5 lc rgb "red" w p, \
	"" every ::3::5  u (log10($$1/abar)):($$2/$$3) t "" pt 13 ps 1.5 lc rgb "magenta" w p\
	;' > $(out)

fig4_2.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set key bottom;\
	set xlabel "$$r/r_\\\\textrm{min}$$";\
	set ylabel "$$V(r)/\\\\epsilon_0$$";\
	Rc = 1;\
	C6 = 1;\
	h(x)=(x>=0?1.0:0.0);\
	V6(r,rc)=-C6/r**6*h(r-rc)+h(rc-r);\
	R0 = Rc*0.88;\
	Rmin = Rc*1;\
	V10(r,rmin)=(3*(rmin/r)**10-5*(rmin/r)**6)/2;\
	V10b(r,r0)=sqrt(5**5/4/3**3)*((r0/r)**10-(r0/r)**6);\
	Morse(r,r0,rmin)=4*(4**(-(r-r0)/(rmin-r0))-2**(-(r-r0)/(rmin-r0)));\
	set samples 300;\
	plot[0.7:2.5][-1.2:0.2] \
	V6(x,Rc) t "Van der Waals" lt 1 lw 5 lc rgb "#7455AA" w l, \
	Morse(x,R0,Rmin) t "Morse" lt 1 lw 5 lc rgb "#FFA800" w l, \
	V10(x,Rmin) t "Lennard-Jones" lt 1 lw 5 lc rgb "#13D6B3" w l, \
	0*x t "" lt 1 lw 1 lc rgb "black" w l\
	;' > $(out)

fig4_4.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex color; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set fit quiet;\
	set fit logfile "/dev/null";\
	set cbrange [0:5];\
	abar =  0.955977594972250;\
	set xlabel "$$n$$";\
	set ylabel "$$|\\\\aminus|/\\\\vdW$$";\
	#set ylabel "$$\\\\dfrac{\\\\aminus}{\\\\vdW}$$";\
	f1(rc)=A1*rc+B1*rc**2+C1;\
	f2(rc)=A2*rc+B2*rc**2+C2;\
	f3(rc)=A3*rc+B3*rc**2+C3;\
	H(x)=(x<=1) ? sqrt(-1) : 1;\
	A1 = -31.7641;A2 = -31.7641;A3 = -31.7641;\
	B1 = 0.6;B2 = 0.6;B3 = 0.6;\
	C1 = -0.5;C2 = -0.5;C3 = -0.5;\
	i1 = 2;\
	i2 = 12;\
	i3 = 52;\
	fit f1(x) "data/AminusCutDependence2" i 0 u 1:(column(i1)) via A1,B1,C1;\
	fit f2(x) "" i 0 u 1:(column(i2)) via A2,B2,C2;\
	fit f3(x) "" i 0 u 1:(column(i3)) via A3,B3,C3;\
	h(x)=(x>=0?1.0:0.0);\
	s(x)=x*2+1;\
	rc(n)=sqrt(2/(pi*(n+7.0/8)));\
	aminus(n) = 63.512/sqrt(pi*(n+7.0/8));\
	aminus1(n) = -f1(rc(n))*sqrt(2);\
	aminus2(n) = -f2(rc(n))*sqrt(2);\
	aminus3(n) = -f3(rc(n))*sqrt(2);\
	set label "$${}^7$$Li" at 10,6.5;\
	set label "$${}^{39}$$K" at 4,23;\
	set label "$${}^{85}$$Rb" at 14,13;\
	set label "$${}^{133}$$Cs" at 18,13;\
	set arrow from 17.5,12 to 22.5,12 heads size .35,90;\
	set object 2 rect from 0,9.45*0.85 to 25,9.45*1.15 fc rgb "grey";\
	set samples 1000;\
	plot[0:25][0:25] 9.45 t "Mean value $$9.8$$" lt 2 lw 1 lc rgb "black", \
	"data/AtomicData" every ::0::0 u (11):(-$$3/$$2) t "" pt 5 ps 1.5 lc rgb "green" w p, \
	"" every ::1::1 u (s($$5)):(-$$3/$$2) t "" pt 7 ps 1.5 lc rgb "black" w p, \
	"" every ::2::2 u (16):(-$$3/$$2) t "" pt 9 ps 1.5 lc rgb "red" w p, \
	"" every ::3::5 u (2*($$5)+12):(-$$3/$$2) t "" pt 13 ps 1.5 lc rgb "magenta" w p, \
	aminus1(x)*H(17-aminus1(x)) t "Single-channel zero-range" lt 1 lw 3 lc rgb "red", \
	aminus2(x)*H(17-aminus2(x)) t "Two-channel, $$\\\\log(s_\\\\text{res})=0$$" lt 3 lw 3 lc rgb "green", \
	aminus3(x)*H(17-aminus3(x)) t "Two-channel, $$\\\\log(s_\\\\text{res})=-0.7$$" lt 5 lw 3 lc rgb "blue", \
	-1 t ""\
	;' > $(out)

fig5_1.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set size 0.9,0.7;\
	set samples 301;\
	set key bottom right Left width -2;\
	set xlabel "$$\\\\rho/|a|$$";\
	set ylabel "$$\\\\dfrac{\\\\nu_1^2-1/4}{(\\\\rho/a)^2}$$";\
	#set label "$$\\\\times10^3$$" at graph 0.9,-.2;\
	# Draw the incoming wave function and the corresponding outgoing splitting \
	YY = 0.78;\
	set label "$$f(\\\\rho) = He^{-ik\\\\rho}+Ge^{ik\\\\rho}$$" at graph .45,YY+0.05;\
	set arrow from graph 0.10,YY to graph 0.98,YY lt 1 lw 3 lc rgb "black" nohead;\
	set arrow from graph 0.05,YY-0.1 to graph 0.05,YY-0.2 size 4,2 lt 1 lw 3 lc rgb "black";\
	set arrow from graph 0.10,YY+0.15 to graph 0.20,YY+0.15 size 4,2 lt 1 lw 3 lc rgb "black";\
	set arrow from 0.70,-0.175 to 0.70,0 lt 1 lw 1 lc rgb "blue" nohead;\
	#Draw the virtual states in the potentials \
	set arrow from graph 0.0,0.25 to graph 0.15,0.25 lt 1 lw 6 lc rgb "green" nohead;\
	set arrow from graph 0.0,0.48 to graph 0.165,0.48 lt 1 lw 6 lc rgb "green" nohead;\
	set arrow from graph 0.0,0.70 to graph 0.195,0.70 lt 2 lw 6 lc rgb "red" nohead;\
	xmin = 0; xmax = 5; ymin = -0.2; ymax = .2; Vmin = -.15;\
	g(y) = (y-1.0/4)/(2*$$1**2);\
	f(y) = g(y)*((g(y)<Vmin)?0:1)+((g(y)<Vmin)?Vmin:0);\
	transX(x) = xmin+(xmax-xmin)*x;\
	transY(y) = ymin+(ymax-ymin)*y;\
	set xtics add ("$$r_\\\\textnormal{imag}$$" 0.7);\
	plot[xmin:xmax][ymin:ymax] \
	"data/chap2/lambda.dat" u ($$1):(f($$2)) t "$$V(\\\\rho)$$" lt 1 lw 6 lc rgb "black" w l,\
	"+" u (transX(bezier4(0.1,0.05,0.05,0.05,$$1/xmax))):\
		(transY(bezier4(YY,YY,YY,YY-0.2,$$1/xmax))) t "" lt 1 lw 3 lc rgb "black" w l,\
	"+" u (transX(bezier4(0.1,0.0,0.0,0.1,$$1/xmax))):\
		(transY(bezier4(YY,YY,YY+.15,YY+.15,$$1/xmax))) t "" lt 1 lw 3 lc rgb "black" w l,\
	0 t "" lt 1 lw 1 lc rgb "#000000" w l,\
	d#"+" u (0.84):(0) t "$$\\\\rho_0/|a|=0.84$$" pt 7 lc rgb "red" w p,\
	1 t "Bound state" lt 1 lw 3 lc rgb "green",\
	1 t "Resonance" lt 2 lw 3 lc rgb "red",\
	((x<=0.73)?-0.175:1/0) t "$$V_\\\\textrm{imag}$$" lt 1 lw 6 lc rgb "blue" w l;\
	' > $(out)

fig5_2.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set xlabel "$$|\\\\Vim|\\\\dfrac{m\\\\rim^2}{\\\\hbar^2}$$";\
	plot[:120][] \
	"data/chap6/V0imagDependence3" u 1:2 t "K" lt 1 lw 3 lc rgb "red" w l,\
	"" u 1:3 t "A" lt 1 lw 3 lc rgb "green" w l,\
	"" u 1:6 t "$$\\\\delta$$" lt 1 lw 3 lc rgb "cyan" w l,\
	"" u 1:7 t "B" lt 1 lw 3 lc rgb "blue" w l,\
	"" u 1:10 t "$$\\\\beta$$" lt 1 lw 3 lc rgb "magenta" w l,\
	"" u 1:(1-exp(-4*$$11)) t "$$1-e^{-4\\\\gamma}$$" lt 1 lw 3 lc rgb "black" w l\
	;' > $(out)

fig5_3.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set size 0.9,0.7;\
	set key width -5;\
	set logscale x; set logscale y;\
	set xrange [] reverse;\
	set xlabel "$$a [a_0]$$";\
	set ylabel "$$\\\\rec$$ [cm$$^6/$$s]";\
	set format x "$$-10^{%L}$$";\
	set format y "$$10^{%L}$$";\
	set label sprintf("%.0f K", 0.0) at 4e4,3e-16 right;\
	set label sprintf("%.1f $$\\\\mu$$K", 0.5) at 4e4,37.5e-20 right;\
	set label sprintf("%.1f $$\\\\mu$$K", 1.0) at 4e4, 7.5e-20 right;\
	set label sprintf("%.1f $$\\\\mu$$K", 2.0) at 4e4, 1.5e-20 right;\
	etas = 0.12;as = -250;s0 = 1.006237839;\
	col1 = "#FF0000";\
	col2 = "#0000FF";\
	set arrow from 2657,4e-20 to 2657,0.5e-18 lt 1 lw 3 lc rgb interpRGB(col1,col2,2.0/3) nohead;\
	set arrow from 1879,5e-21 to 1879,0.5e-18 lt 1 lw 3 lc rgb interpRGB(col1,col2,1.0/3) nohead;\
	set arrow from 1328,6e-22 to 1328,0.5e-18 lt 1 lw 3 lc rgb interpRGB(col1,col2,0) nohead;\
	set label "$$\\\\overbrace{\\\\phantom{sums}}$$" at 1897,0.5e-18 center;\
	set label "$$a_C$$" at 1897,0.5e-17 center;\
	y(a) = 4590*sinh(2*etas)/(sin(s0*log(a/as))**2+sinh(etas)**2)*a**4*2.83923e-37;\
	plot [40:2.5e5][1e-26:1e-15]\
	y(-x)*((x<2e4)?1:1/0) t "Braaten \\\\& Hammer" lt 1 lw 5 lc rgb "green" w l, \
	"data/chap6/Li7recombinationPoints.dat" u (-$$1):2 t "$${}^7$$Li @ $$1.5\\\\mu$$K" pt 7 lw 3 lc rgb "purple" w p, \
	"data/chap6/Li7thermalData" u (-$$1):2 t "" lt 1 lw 3 lc rgb "blue" w l, \
	"" u (-$$1):3 t "" lt 1 lw 3 lc rgb interpRGB(col1,col2,2.0/3) w l,\
	"" u (-$$1):4 t "" lt 1 lw 3 lc rgb interpRGB(col1,col2,1.0/3) w l,\
	"" u (-$$1):5 t "" lt 1 lw 3 lc rgb interpRGB(col1,col2,0) w l\
	d#"data/chap6/Li7recombination.dat" u (-$$1):2 t "" lt 1 lw 3 lc rgb "blue" w l, \
	d#"" u (-$$1):10 t "" lt 1 lw 3 lc rgb interpRGB(col1,col2,0) w l,\
	d#"" u (-$$1):11 t "" lt 1 lw 3 lc rgb interpRGB(col1,col2,1.0/3) w l,\
	d#"" u (-$$1):12 t "" lt 1 lw 3 lc rgb interpRGB(col1,col2,2.0/3) w l\
	;' > $(out)

fig5_4.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set size 0.9,0.7;\
	set key bottom left;\
	set logscale x;	set logscale y;\
	set xlabel "$$a [a_0]$$"; set ylabel "$$\\\\gamma$$";\
	col1 = "#FF0000";\
	col2 = "#0000FF";\
	set xtics format "$$-10^{%L}$$";\
	set ytics format "$$10^{%L}$$";\
	T = "1.5358e-04 7.6792e-05 3.8396e-05 1.9198e-05 9.6e-06\
		4.8e-06 2.4e-06 1.2e-06 6e-07 3e-07";\
	plot [3e4:50][:0.99] \
		for [j=3:10] "data/chap6/eta_star_finite_T.dat"\
		i 0 u (-$$1):(column(j))\
		t sprintf("%3.1f $$\\\\mu$$K", word(T,j-1)*1e6)\
		lt 1 lw 3 lc rgb interpRGB(col1,col2,(j-2.0)/9) w l\
	;' > $(out)

fig5_5.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set logscale x; set logscale y;\
	set xrange [] reverse;\
	set xlabel "$$a [a_0]$$"; set ylabel "$$\\\\rec$$ [cm$$^6/$$s]";\
	set format x "$$-10^{%L}$$";\
	set format y "$$10^{%L}$$";\
	set label sprintf("%.0f K", 0)     at 8.7e4,1.00e-16 right;\
	set label sprintf("%.0f nK", 1)    at 8.7e4,0.5e-17right;\
	set label sprintf("%.0f nK", 4)    at 8.7e4,0.5e-18right;\
	set label sprintf("%.0f nK", 15)   at 8.7e4,0.33e-19 right;\
	set label sprintf("%.0f nK", 60)   at 8.7e4,1.9e-21 right;\
	set label sprintf("%.0f nK", 240)  at 8.7e4,1.1e-22 right;\
	#set label sprintf("%.0f K", 0)      at 8.7e4,1.00e-16 right;\
	#set label sprintf("%.0f nK", 2)     at 8.7e4,1.76e-18 right;\
	#set label sprintf("%.0f nK", 8)     at 8.7e4,1.27e-19 right;\
	#set label sprintf("%.0f nK", 40)    at 8.7e4,5.12e-21 right;\
	#set label sprintf("%.0f nK", 170)   at 8.7e4,2.70e-22 right;\
	set ytics 1e-24,100,1e-16;\
	etas = 0.12;as = -250;s0 = 1.006237839;\
	y(a) = 4590*sinh(2*etas)/(sin(s0*log(a/as))**2+sinh(etas)**2)*a**4*2.83923e-37;\
	H(x,a) = (x>a)?1:1/0;\
	# Fancy interpolation between two colors;\
	col1 = "#FF0000";\
	col2 = "#0000FF";\
	plot [100:5e5][1e-25:5e-16]\
	"data/chap6/Cs133recombination.dat" i 3 u (-$$1):2 t "853.07 G" pt 13 ps 1.5 lc rgb "blue" w p,\
	"" i 2 u (-$$1):2 t "554.71 G" pt 7 ps 1.5 lc rgb "green" w p,\
	"" i 1 u (-$$1):2 t "553.3 G" pt 9 ps 1.5 lc rgb "red" w p,\
	"data/chap6/Cs133Thermal2" u (-$$1):($$2*H($$1,-4e4)) t ""\
			lt 1 lw 3 lc rgb interpRGB(col1,col2,1.0) w l,\
	"" u (-$$1):($$3*H($$1,-8e4)) t ""\
			lt 1 lw 3 lc rgb interpRGB(col1,col2,0.8) w l,\
	"" u (-$$1):($$4*H($$1,-8e4)) t ""\
			lt 1 lw 3 lc rgb interpRGB(col1,col2,0.6) w l,\
	"" u (-$$1):($$5*H($$1,-8e4)) t ""\
			lt 1 lw 3 lc rgb interpRGB(col1,col2,0.4) w l,\
	"" u (-$$1):($$6*H($$1,-8e4)) t ""\
			lt 1 lw 3 lc rgb interpRGB(col1,col2,0.2) w l,\
	"" u (-$$1):($$7*H($$1,-8e4)) t ""\
			lt 1 lw 3 lc rgb interpRGB(col1,col2,0.0) w l \
	;' > $(out)

fig6_2.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set samples 301;\
	set key Left width 0;\
	set xlabel "$$\\\\left[\\\\dfrac{\\\\rho}{|a|}+1\\\\right]\\\\sqrt{2\\\\R}-\\\\dfrac{\\\\R}{\\\\sqrt{2}}$$";\
	set ylabel "$$\\\\dfrac{\\\\nu^2-1/4}{\\\\R\\\\rho^2}$$";\
	plot[0:6][-0.3:1] \
	"data/chap7/massImbalancedPotentials" u ($$1):($$2) t "$$\\\\R=0.1$$" lt 1 lw 3 lc rgb "red" w l,\
	"" u ($$3): ($$4)  t "$$\\\\R=0.2$$" lt 1 lw 3 lc rgb "green" w l,\
	"" u ($$5): ($$6)  t "$$\\\\R=0.5$$" lt 1 lw 3 lc rgb "blue" w l,\
	"" u ($$7): ($$8)  t "$$\\\\R=1$$"   lt 1 lw 3 lc rgb "cyan" w l,\
	"" u ($$9): ($$10) t "$$\\\\R=5$$"   lt 1 lw 3 lc rgb "magenta" w l,\
	"" u ($$11):($$12) t "$$\\\\R=10$$"  lt 1 lw 3 lc rgb "yellow" w l,\
	0 t "" lt 1 lw 1 lc rgb "black"' > $(out)

fig6_3.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set samples 301;\
	set key Left width -6;\
	set xlabel "$$\\\\dfrac{\\\\rho}{|a|}$$";\
	set ylabel "$$\\\\dfrac{\\\\nu^2-1/4}{\\\\rho^2}$$";\
	xmin =  0; xmax = 10; ymin = -2; ymax =  4; Vmin = -1.5;\
	T    = 24690383.7249007;\
	g(y) = T*(y+15.0/4)/(2*$$1**2);\
	f(y) = g(y)*((g(y)<Vmin)?0:1)+((g(y)<Vmin)?Vmin:0);\
	transX(x) = xmin+(xmax-xmin)*x;\
	transY(y) = ymin+(ymax-ymin)*y;\
	plot[0:20][-0.2:0.5] \
	"data/chap7/massImbalancedPotentials3" \
	   u ($$1):($$2) t "$$\\\\R=0.1$$"       lt 1 lw 3 lc rgb "red"     w l,\
	"" u ($$1):($$3) t "$$\\\\R=0.2084$$"    lt 1 lw 3 lc rgb "green"   w l,\
	"" u ($$1):($$4) t "$$\\\\R=0.5$$"       lt 1 lw 3 lc rgb "blue"    w l,\
	"" u ($$1):($$5) t "$$\\\\R=1$$"         lt 1 lw 3 lc rgb "cyan"    w l,\
	"" u ($$1):($$6) t "$$\\\\R=5$$"         lt 1 lw 3 lc rgb "magenta" w l,\
	"" u ($$1):($$7) t "$$\\\\R=10$$"        lt 1 lw 3 lc rgb "yellow"  w l,\
	"" u ($$1):($$8) t "Identical particles" lt 1 lw 3 lc rgb "black"   w l,\
	15.0/8/x/x t "$$15/(4\\\\rho^2)$$" lt 2 lw 3 lc rgb "black" w l, \
	0 t "" lt 1 lw 1 lc rgb "black"' > $(out)

fig6_4.gnu:
	@$(eval out = $(figurefolder)/$@)
	@echo \
	'set term epslatex; set out "$(figurefolder)/$(@:.gnu=.tex)";\
	set size $(figuresize);\
	set logscale x; set logscale y;\
	set xrange [] reverse;\
	set xlabel "$$a [a_0]$$"; set ylabel "$$\\\\rec$$ [cm$$^6/$$s]";\
	set format x "$$-10^{%L}$$";\
	set format y "$$10^{%L}$$";\
	T = " 8.9996e-05   4.4998e-05   2.2499e-05   1.1250e-05   5.6248e-06   2.8124e-06   1.4062e-06   7.0309e-07   3.5155e-07   1.7577e-07   8.7887e-08   4.3943e-08 2.1972e-08   1.0986e-08   5.4929e-09   2.7465e-09 ";\
	set for[i=1:10:2] label sprintf("%4.1f",word(T,i)*1e6) at 4.5e4,4**-(40-i) right;\
	set for[i=11:16:2] label sprintf("%4.1f",word(T,i)*1e9) at 4.5e4,4**-(40-i) right;\
	set for[i=1:10:2] label sprintf("$$\\\\mu$$K",word(T,i)*1e6) at 4e4,4**-(40-i);\
	set for[i=11:16:2] label sprintf("nK") at 4e4,4**-(40-i);\
	set label 18 sprintf("%4.0f",0) at 4.5e4,1e-14 right;\
	set label 28 sprintf("K") at 3.35e4,1e-14 ;\
	etas = 0.12;as = -250;s0 = 1.006237839;\
	y(a) = 4590*sinh(2*etas)/(sin(s0*log(a/as))**2+sinh(etas)**2)*a**4*2.83923e-37;\
	H(x) = (x>0)?1:1/0;\
	col1 = "#FF0000";\
	col2 = "#0000FF";\
	plot [][:1e-13]\
	"data/chap7/CsLiRecombination2.dat" i 0 u (-$$1):2 t "" lt 1 lw 3 lc rgb "blue" w l,\
	for [j=3:17:2] "" i 0 u (-$$1):(column(j)*H(2e4+$$1)) t "" lt 1 lw 3 lc rgb interpRGB(col1,col2,(j-3)/18.0) w l\
	;' > $(out)

clean:
	rm -f *.aux *.dvi *.log *.out *.ps *.bbl *.log *.blg\
		*.gnu *.auxlock *.gz *.lot *.lof *.toc figures/*.gnu\
		$(addprefix figures/,$(FIGURES:=.tex))\
		$(addprefix figures/,$(FIGURES:=.eps))


==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_PROGRAM_AUTHOR	Darren Hiebert	/dhiebert@users.sourceforge.net/
!_TAG_PROGRAM_NAME	Exuberant Ctags	//
!_TAG_PROGRAM_URL	http://ctags.sourceforge.net	/official site/
!_TAG_PROGRAM_VERSION	5.9~svn20110310	//
Acknowledgements	acknowledgements.tex	/^yderligere information om de fysiske vekselvirkninger.$/;"	c
Adaptive step size	appendixA.tex	/^which is easily calculated at a low extra cost in computation.$/;"	b
Bound trimers	chapter3.tex	/^\\fig{figure:3.2}.$/;"	s
Cold atoms and recombination	chapter1.tex	/^atoms~\\cite{kraemer2006,ferlaino2010}.$/;"	s
Comparison to experiment	chapter3.tex	/^\\end{figure}$/;"	s
Comparison to experimental data	chapter5.tex	/^\\end{figure}$/;"	s
Conclusion	chapter5_old.tex	/^concerning its position of the second minimum.$/;"	s
Conclusions	chapter3.tex	/^\\end{figure}$/;"	s
Conclusions	chapter5.tex	/^be required to observe this peak clearly.$/;"	s
Conclusions	chapter6.tex	/^from \\fig{figure:5.3}.$/;"	s
Dansk	acknowledgements.tex	/^into the universal theories.$/;"	s
Effective range expansion	chapter2.tex	/^support yet another bound state with energy zero.$/;"	u
Effective range expansion model  hyper-spherical edition	chapter2.tex	/^one still needs to introduce a short-distance cut-off.$/;"	u
Efficiently solving the eigenvalue equations	appendixA.tex	/^% VIM: let b:latex_main="main.pdf"$/;"	c
Efimov and Thomas effects	chapter2.tex	/^where $s_0=1.0062378$ whereas the next solution is $\\nu_1=4.46529$.$/;"	u
English	acknowledgements.tex	/^\\chapter{Resume \/ Resumé}$/;"	s
Experimental comparison	chapter5_old.tex	/^% VIM: let b:latex_main="main.pdf"$/;"	c
Feshbach resonances	chapter1.tex	/^for current experiments.$/;"	s
Feshbach resonances	chapter2.tex	/^function has to be normalizable.$/;"	u
Few-body physics and the Efimov effect	chapter1.tex	/^\\label{introduction1}$/;"	s
Finite range effects	chapter3.tex	/^% VIM: let b:latex_main="main.pdf"$/;"	c
Finite range effects	chapter5_old.tex	/^resonances.$/;"	s
Finite-range effects in the recombination rate	chapter3.tex	/^seen for all cut-offs, however with different absolute values.$/;"	s
Hyper-spherical coordinates	chapter2.tex	/^still be applied.$/;"	u
Introduction	chapter1.tex	/^% VIM: let b:latex_main="main.pdf"$/;"	c
Low-energy limit of recombination probability	appendixB.tex	/^% VIM: let b:latex_main="main.pdf"$/;"	c
Mass-imbalanced systems	chapter6.tex	/^% VIM: let b:latex_main="main.pdf"$/;"	c
Methods of describing three-body physics	chapter1.tex	/^increased.$/;"	s
Model Comparison	chapter3.tex	/^investigated further in the next chapter.$/;"	s
Positive effective range	chapter2.tex	/^precisely as in \\eqr{eq:2.80}.$/;"	b
Properties of the mass-imbalanced potentials	chapter6.tex	/^reduced mass of this subsystem and $\\phi=\\phi_{12}$ from \\eqr{eq:2.51}.$/;"	u
Quadratic extrapolation	appendixA.tex	/^section \\ref{hidden_crossing_theory}.$/;"	b
Recombination for negative scattering lengths	chapter5.tex	/^% VIM: let b:latex_main="main.pdf"$/;"	c
Results	chapter6.tex	/^the mixed Cs-Li system compared to a system of identical particles.$/;"	s
Resume  Resum  	acknowledgements.tex	/^% VIM: let b:latex_main="main.pdf"$/;"	c
Summary and Outlook	chapter7.tex	/^% VIM: let b:latex_main="main.pdf"$/;"	c
Temperature effects	chapter5.tex	/^\\end{figure}$/;"	u
The Efimov effect as indirect observation	chapter1.tex	/^experimental set-ups \\cite{esry1999, Macek1999, braaten2001}.$/;"	s
The mass-imbalanced eigenvalue equation	chapter6.tex	/^initial investigation phase.$/;"	s
The optical model	chapter5.tex	/^limit \\cite{dincao2004}.$/;"	s
The recombination coefficient	chapter5.tex	/^models.$/;"	s
The short distance limit	chapter2.tex	/^energy of the dimers.$/;"	b
The two-channel model	chapter2.tex	/^channels.$/;"	u
The two-channel model relation to Feshbach resonances	chapter2.tex	/^effective range is always negative \\cite{chin2010}.$/;"	b
The zero-range model	chapter2.tex	/^between $\\pm\\infty$, the effective range, $R$, will vary much less.$/;"	u
The zero-range model  hyper-spherical edition	chapter2.tex	/^\\end{equation}$/;"	u
Theory and Methods	chapter2.tex	/^% VIM: let b:latex_main="main.pdf"$/;"	c
Thesis outline	chapter1.tex	/^schmidt2012}.$/;"	s
Three-body parameter	chapter1.tex	/^retaining computational simplicity and interpretative elegance.$/;"	s
Three-body physics	chapter2.tex	/^two-channel model through \\eqrs{eq:2.32}.$/;"	s
Three-body recombination rate	chapter2.tex	/^relevant).$/;"	s
Threshold for trimer creation	chapter3.tex	/^usual Efimov scaling factor.$/;"	u
Trimer threshold value revisited	chapter4.tex	/^ranges, and range effects are thus hard to see in these systems.$/;"	s
Two-body physics	chapter2.tex	/^methods, implemented on top of these models, are presented.$/;"	s
Two-body potentials	chapter4.tex	/^\\cite{chin2010}, so the here presented method is preferable.$/;"	s
Two-body scattering	chapter2.tex	/^\\label{two_body_physics}$/;"	u
Two-channel model  hyper-spherical edition	chapter2.tex	/^its inclusion.$/;"	u
Universal Three-Body Parameter	chapter4.tex	/^% VIM: let b:latex_main="main.pdf"$/;"	c
appendixA	main.tex	/^\\appendix$/;"	i
appendixB	main.tex	/^\\include{appendixA}$/;"	i
chapter1	main.tex	/^\\mainmatter$/;"	i
chapter2	main.tex	/^\\include{chapter1}$/;"	i
chapter3	main.tex	/^\\include{chapter2}$/;"	i
chapter4	main.tex	/^\\include{chapter3}$/;"	i
chapter5	main.tex	/^\\include{chapter4}$/;"	i
chapter6	main.tex	/^\\include{chapter5}$/;"	i
chapter7	main.tex	/^\\include{chapter6}$/;"	i

